A Safety Assurable Human-Inspired Perception Architecture

Although artificial intelligence-based perception (AIP) using deep neural networks (DNN) has achieved near human level performance, its well-known limitations are obstacles to the safety assurance needed in autonomous applications. These include vulnerability to adversarial inputs, inability to handle novel inputs and non-interpretability. While research in addressing these limitations is active, in this paper, we argue that a fundamentally different approach is needed to address them. Inspired by dual process models of human cognition, where Type 1 thinking is fast and non-conscious while Type 2 thinking is slow and based on conscious reasoning, we propose a dual process architecture for safe AIP. We review research on how humans address the simplest non-trivial perception problem, image classification, and sketch a corresponding AIP architecture for this task. We argue that this architecture can provide a systematic way of addressing the limitations of AIP using DNNs and an approach to assurance of human-level performance and beyond. We conclude by discussing what components of the architecture may already be addressed by existing work and what remains future work.

==> notes.tex <==


Second, a classifier  However, performance should be compared conditioned on the difficulty of the cases for a human. In particular, the cases that are easy for humans should be easy for the \aip. Adversarial examples violate this condition. A simple way to achieve this is to partition class into [this is trickier than this - I want to capture the fact that the embodiment prior makes some case variations easier - metamorphic relations.]
[performance comparisons of \aip~to humans should be measured according to human-based ``hardness'']
    \begin{itemize}
        \item species fair comparisons~\cite{firestone2020performance}. The idea is that when we compare humans to machines and find that their performance is different we shouldn't necessarily assume this is due to their inherent competency because it could be a constraint of their operational environment. For example, the retina is high resolution in the centre (fovea) but loses resolution and is color blind at the periphery. Thus, it sees an image differently than a DNN that gets an image as a uniform pixel grid. This difference can result in different classification accuracy of an image even if this has nothing to do with classification knowledge. One fix is to constrain the DNN to see the image the way a human would. For example, one train a DNN prepended with a transformation that distorts and image the retina would. Researchers found that in this kind of setup, adversarial examples for the DNN turned out to fool humans too, when under time pressure~\cite{elsayed2018adversarial}. Also see~\cite{geirhos2020beyond}.  
        \item comparisons should be risk-aware - performance differences in a context that is not safety relevant is not important. E.g., 
        \item time is a factor - the performance similarity at a given speed is important. Or more broadly, Type 1 should be compared to Type 1 and Type 2 to Type 2
        \item invariances of easy cases are still easy
        \item basic-level classification is easier than super or subordinate level 
        \item Hard cases for humans could also be hard for ADS, but cautionary principle used for safety

    \end{itemize}

\section{notes}
In particular, these concepts are meaningful for assessing the situational risk of different behavioural decisions humans can make during driving --- i.e., humans know what harms might happen to various objects as a consequence of their driving and how much to care about this. This risk perception is especially important for novel objects that are difficult to classify. 

Second, these concepts are typically not explicitly ``defined'' but rather they emerge through an imperfect process of implicit social consensus. This has various implications. The concept can vary across communities affecting the transferability of knowledge --- e.g., what is considered a typical cyclist in Canada may be different than in Vietnam. Even people in a given community may reasonably disagree about the classification of specific ambiguous cases, which means that some examples have no well-defined ground truth. The concept also naturally changes over time, e.g., as new types of cyclist vehicles are invented, exhibiting distributional shift.
\subsection{Objectives/topics/Contributions}
\begin{itemize}
    \item That DNNs have deficiencies is a common concern (Goyal, etc.) Examples are given (inability to deal with novelty, adversarial inputs, non-interpretability) but the reasons why these problems exist are not well articulated. Although some give reasons such as disconnection in a distributed representation, lack of compositionality, ... The reasons are in terms of operational deficiencies of the NN. Instead, we give reasons in terms of the characteristics of the classification problem itself (insufficiency of visual feature representation because of conceptual nature of class), the physical process (confounding impacts of image-taking on class - although is this really a reason why DNNs are not enough?) and the assurance problem (a:for human baseline comparisons, performance should not be measured generally but broken down by hardness categories (doesn't KITTI do this?) - in particular, the easyness of invariants that are common to humans and typical examples (scoped by community and time), as opposed to exposure to atypical examples that could vary among humans; b: compositionality of evidence from architectural alignments with how humans do it; c: the non-interpretability of DNNs can be addressed by factoring out certain non-interpretable but reusable functionality that (may be) class-agnostic (specifically, object normalization and similarity assessment) from class-specific (intrepretable classification of normalized object using exemplar/prototype approaches))
    \item Topic: the limits of CV ML classification 
    \item Topic: A safe human-inspired classification architecture
    \begin{itemize}
        \item Rather than promoting a particular architecture, I want to claim that humans use a dual process architecture because it is actually necessary 
        \begin{enumerate}
            \item to address classes like Cyclist - there are limitations with visual features used in Type 1
            \item to address the speed/accuracy trade-off needed for fast safety-critical decisions - i.e., for very fast decisions a Type 2 conscious reasoning approach would be too slow (and the decision should be conservative - but I don't have support for this aspect). But why is conscious reasoning necessarily slow? 1) intuition: compilation; 2) the speed of reasoning is dependent on the bound on knowledge being accessed - type 2 has access to all of conceptual knowledge (although it doesn't follow that it always has to use it - i.e., it could access it in a graduated way according to available time); 3) the visual sense domain is distinct from the conceptual domain in the sense that what is reified in the former do not correspond to concepts in the realm of social discourse  
            \item since all information about the world is only available through sense data which is mediated by type 1 mechanisms (e.g., symbol grounding problem), type 2 reasoning is dependent on type 1 processes. I need a nice example of the unbounded problem of type 1 processes necessitating type 2. Ideally, even a general argument (proof) that looks something like this: say that there is some set of visual features necessary and sufficient to charcterize a classification problem. I claim there is always another feature, that in some context, is necessary to assess for the classification (i.e., an example will satisfy the visual features for C and yet will be notC (i.e., FP) or conversely (i.e., FN)). Well I can't prove it but there are convincing arguments: a) non-observable but conceptually relevant features - e.g., bike frame made out of a material that is not stable - but eventually some kind of test must be doable that allows for an observation. This where it connects to philosophy of science - checking conceptual features must ultimately correspond to checking some observable (i.e., visual) features otherwise it the classificiation is unscientific - scientifically ``undecidable'' - although, another possibility is that the maker of the bike (authorative source) asserts that it is made using an unstable material - unlike science we are classifyng artifacts as well as natural kinds; b) the issue of disguises or mimics, malicious or otherwise. 
        \end{enumerate}
        \item The decomposition of the classification problem allows a corresponding decomposition of the argument. Specifically, we decomposes the classification problem by first normalizing objects subtracting out elements that humans consider irrelevant to class and then it classifies the normalized object either using a DNN or symbolic AI if too low confidence
        \item Aligning this decomposition architecture with how humans do it provides a basis for evidence that it does it as well as humans. Specifically, it allows us to compare the performance of the different stages to the corresponding human stage, separately. If the architectures were different, we could only make comparisons at the whole classification level (black box). So this allows a grey-box comparison. 
        \item (very important) Another assurance factor is that the ``hardness'' level of an input (i.e., how hard it is to classify) should align with human opinion. A system that calls something hard that humans consider easy is alien and less trustworthy. This factor is hidden by performance metrics - i.e., they only give performance averaged over all cases but have the same metric value does not mean that it performs the same as humans on the same cases! What we want in a human baseline is to have the same as human performance at every hardness level (as judged by humans). 
    \end{itemize}
\end{itemize}

\subsection{Parts}
\begin{itemize}
    \item Classification task during driving
        \begin{itemize}
            \item Classification as a fundamental (atomic) perception task
            \item Distinction between object vs object image classification. 
            \item Do I need a section on image taking? This is relevant in a number of places
            \begin{itemize}
                \item Embodied learning
                \item The definition of identity and classification invariants
                \item The limits of object image classification (and therefore, of CV ML classification with or without help) due to uncertainty in the O2I function
            \end{itemize}
        \end{itemize}

    \item Assurance objective for ADS
    \begin{itemize}
        \item We introduce a human baseline (a lower bound for safety) for classification performance as the Status Quo Assurance Assumption
        \item One counter to this is that maybe the human baseline on safe activity is only relevant at the whole perception subsystem level or whole ADS level - i.e., individual components need to carry out tasks as well as humans if this is compensated for at the system level. Although this is valid, having a human baseline at the component task level is a conservative goal and it is worth asking if it is achievable.
    \end{itemize}
\end{itemize}
